Partial bases and homological stability of $\operatorname{GL}_{n}(R)$ revisited

Let $R$ be a unital ring satisfying the invariant basis number property, that every stably free $R$-module is free, and that the complex of partial bases of every finite rank free module is Cohen--Macaulay. This class of rings includes every ring of stable rank $1$ (e.g. any local, semi-local or Artinian ring), every Euclidean domain, and every Dedekind domain $\mathcal{O}_S$ of arithmetic type where $|S| > 1$ and $S$ contains at least one non-complex place. Extending recent work of Galatius--Kupers--Randal-Williams and Kupers--Miller--Patzt, we prove that the sequence of general linear groups $\operatorname{GL}_n(R)$ satisfies slope-$1$ homological stability with $\mathbb{Z}[1/2]$-coefficients.

==> latex-config/packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage[backend=bibtex, style=alphabetic, url=false, hyperref, backref, backrefstyle=none, maxbibnames=99, sorting=nyt, safeinputenc]{biblatex}
\AtEveryBibitem{\clearlist{language}}
\addbibresource{sources.bib}
\renewcommand*{\bibfont}{\small}
\RequirePackage{doi}

\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{stix}
\usepackage{stmaryrd}
\usepackage{array}

\usepackage{tikz}
\usepackage{tikz-cd}

\usepackage{xparse}
\usepackage{etoolbox}
\usepackage{aliascnt}
\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
\hypersetup{
	colorlinks=true,
	linkcolor=blue,
	filecolor=blue,
	citecolor = blue,
	urlcolor=blue,
	bookmarksdepth=3,
}
\usepackage[capitalize,nameinlink,noabbrev]{cleveref}
\crefrangelabelformat{equation}{(#3#1#4 -- #5#2#6)}
\crefname{property}{Property}{Properties}
\crefname{claim}{Claim}{Claims}

\usepackage{amsthm}
\usepackage{latex-config/environments}

\usepackage[textsize = footnotesize]{todonotes}
\setlength{\marginparwidth}{2.5cm}

